MemoRec: A Recommender System for Assisting Modelers in Specifying Metamodels

Model Driven Engineering (MDE) has been widely applied in software development, aiming to facilitate the coordination among various stakeholders. Such a methodology allows for a more efficient and effective development process. Nevertheless, modeling is a strenuous activity that requires proper knowledge of components, attributes, and logic to reach the level of abstraction required by the application domain. In particular, metamodels play an important role in several paradigms, and specifying wrong entities or attributes in metamodels can negatively impact on the quality of the produced artifacts as well as other elements of the whole process. During the metamodeling phase, modelers can benefit from assistance to avoid mistakes, e.g., getting recommendations like meta-classes and structural features relevant to the metamodel being defined. However, suitable machinery is needed to mine data from repositories of existing modeling artifacts and compute recommendations. In this work, we propose MemoRec, a novel approach that makes use of a collaborative filtering strategy to recommend valuable entities related to the metamodel under construction. Our approach can provide suggestions related to both metaclasses and structured features that should be added in the metamodel under definition. We assess the quality of the work with respect to different metrics, i.e., success rate, precision, and recall. The results demonstrate that MemoRec is capable of suggesting relevant items given a partial metamodel and supporting modelers in their task.

==> src/Challenges.tex <==


%\smallskip
%\textbf{RQ$_3$: What kind of business logic is most suitable for an LCD platform?} Together with \textbf{RQ$_1$}, this aims at identifying a suitable model for the proposed LCD platform. A possible solution is represented by a domain system language(DSL) that allows the creation, specification, and maintenance of the domain. Thus, new constrains or upcoming changes of the platform are addressed flexibly and easily. 

%\smallskip
%\textbf{RQ$_3$: How is it possible to integrate components of an RSSE into the 
%platform?} This challenge requires the creation of a knowledge base that 
%enables innovative features. The LCD platform must adapt itself to different 
%RSSEs with common skeleton supported by the state of the art contribution

%\smallskip
%\textbf{RQ$_4$: How can the platform support the user's experience? }
%The user experience must be addressed properly to make incisive the LCD 
%platform. A very promising approach is the drag and drop interfaces, as they 
%are well-known by the end-users.

==> src/Modeling.tex <==
\subsection{Design features of Recommender Systems}\label{sec:feature}

According to Robillard \etal~\cite{robillard_recommendation_2014}, any recommender system in software engineering consists of four main activities:
%Recommendation systems are very complex, we have to simplify their 
%representation. To this end, we can 
%isolate four main components involved in the development of a recommender 
%system by examining the 
%plethora 
%of approaches in the literature:

\begin{description}
	\item[Data Preprocessing] In this phase techniques and tools are applied to 
	extract valuable information from different data sources, \eg AST parsing, text mining, and 
	natural language processing;
	
	\item[Capturing Context] Subsequently, the developer context is excerpted 
	from the programming environment to create the recommendation query. Depending on the RSSE, it 
	can be triggered pro-actively or reactively;
	
	\item[Producing Recommendations] The actual recommendation algorithms are chosen and executed to produce hints that are relevant for the current development 
	task. Possible recommendation approaches that can be employed at this stage can be for example model-based, memory-based, make use of filtering techniques, or based on some domain-specific heuristics;
	
	\item[Presenting Recommendations] As the last phase, the produced recommendation items are to be presented to the developer for instance directly in the IDE being used or in an external Web application.
\end{description}

%\vspace{-.1cm}

%\noindent
%\textbf{Data Preprocessing}: In this phase techniques and tools are applied to 
%extract valuable information from different data sources, \eg AST parsing, text mining, and 
%natural language processing;
%
%\noindent
%\textbf{Capturing Context} Subsequently, the developer context is excerpted 
%from the programming environment to create the recommendation query. Depending on the RSSE, it 
%can be triggered pro-actively or reactively;
%
%\noindent
%\textbf{Producing Recommendations} In this phase, the actual recommendation algorithms are chosen and executed to produce hints that are relevant for the current development 
%task. Possible recommendation approaches that can be employed at this stage can be for example model-based, memory-based, make use of filtering techniques, or based on some domain-specific heuristics;
%
%\noindent
%\textbf{Presenting Recommendations} As the last phase, the produced recommendation items need to be properly presented to the developer for instance directly in the IDE being used or in an external Web application.

%%\begin{description}
%\noindent
%{\bf - Data Preprocessing} In this phase techniques and tools are applied to 
%extract valuable 
%information from different data sources, \eg AST parsing, text mining, and 
%natural language processing;
%
%\noindent
%{\bf - Capturing Context} Subsequently, the developer context is excerpted 
%from the programming 
%environment to create the recommendation query. Depending on the RSSE, it 
%can be triggered proactively 
%or reactively;
%
%\noindent
%{\bf Producing Recommendations} In this phase, the actual recommendation 
%algorithms are chosen and 
%executed to produce hints that are relevant for the current development 
%task. Possible recommendation 
%approaches that can be employed at this stage can be for example model-based, 
%memory-based, make use of 
%filtering 
%techniques, or based on some domain-specific heuristics;
%
%\noindent
%{\bf Presenting Recommendations} As the last phase, the produced recommendation 
%items need to be properly 
%presented to the developer for instance directly in the IDE being used or 
%in an external Web 
%application.
%%\end{description}

\revised{By adhering the principles and the methods underpinning the 
development of \rs 
\cite{isinkaye_recommendation_2015,laser_software_2015,bobadilla_recommender_2013},
 such high-level phases 
have been further investigated with the aim of defining interrelated 
\emph{features}~\cite{benavides_automated_2010} as shown in 
Fig.~\ref{fig:featureModel}. For each activity (represented as boxes), 
corresponding features (and sub-features) are depicted as ovals to represent 
possible techniques that can be employed. Due to space limit, the model does 
not represent the relationships among features as well as possible constraints 
governing their usage. Dashed boxes represent attributes of the mandatory 
features to include more information about them, \eg data preprocessing can be employed on source code, Q\&A items like \SO posts, \etc}

%\smallskip
%Figure \ref{fig:featureModel} represents the proposed model, which depicts the 
%most common strategies 
%using in this domain. We represent the four main RSSE components identified by 
%\cite{robillard_recommendation_2014} as mandatory features by adding 
%attributes to better describe some 
%of 
%them \ie the data preprocessing possible inputs. For each entity, we describe 
%instances of approaches 
%exploring possible sub-feature. 

\begin{figure*}[h]
    \centering    
    \includegraphics[width=0.8\linewidth]{figs/featureModel.pdf}
    \vspace{-.5cm}
    \caption{Design features of \rs in software engineering.}
    \label{fig:featureModel}

\end{figure*}


\begin{table*}[h]
    \footnotesize
    \centering
    \begin{tabular}{ | l | l|l |l | l |}  \hline            
        {\bf Recommendation system} & {\bf Data preprocessing} & {\bf Capturing context} & {\bf Producing recommendation}  &  {\bf Presenting recommendation} \\ \hline        
        Strathcona~\cite{holmes_strathcona_nodate}  & AST parsing  & Keyword 
        extraction & Six heuristic functions & IDE integration \\ \hline    
        %+Traversable graph     
        
		Sourcerer~\cite{linstead_sourcerer:_2009} & AST parsing & Indexing & 
		Custom ranking scheme (Heuristic) & Web interface\\ \hline %+Code 
		%Snippets

		\FaC~\cite{kim_f_2018} & AST parsing & Indexing & Alternate query 
		(Heuristic) & Web interface \\ \hline %+Code snippets

		\PR~\cite{ponzanelli_prompter:_2016} & NLP & Indexing & Custom 
		ranking model (Heuristic) & IDE integration\\ \hline   %+ List of posts 

		\rowcolor{verylightgray}
		\CS~\cite{8498236} & Graph representation  & Feature 
		extraction  & Content-based filtering  &  Web integration\\ \hline  
				
		%Similarity project

		\rowcolor{verylightgray}	
		\CR~\cite{NGUYEN2020110460} &Graph representation & Feature 
		extraction & Collaborative filtering  & IDE integration \\ \hline   
		
		
		\rowcolor{verylightgray}
		\FC~\cite{Nguyen:2019:FRS:3339505.3339636} & Tensor & API calls extraction & 
		Context-aware collaborative filtering & IDE integration \\ \hline   %List of API 
		%function call 
		
		
		\rowcolor{verylightgray}
		\AU~\cite{8906979} & NLP  & Feature 
		extraction  & Feed forward neural network  &  Web interface\\ \hline  
		
		%List of libraries 
    \end{tabular}
    \caption{\revised{Characterizing \rs with respect to features.}}
    \label{tab:rsseFeatures}
   	\vspace{-.4cm}
\end{table*}


%EU Horizon 2020 is a research program in which new technologies and approaches are proposed considering their possible scientific innovations. Considering this landscape, CROSSMINER \cite{nguyen_enabling_2019} has been proposed to support the development of complex software systems by facilitating the comparison and the adoption of existing open-source software components. 
%%Thus, we consider the CROSSMINER platform as a particular instance compliant with the feature model. In particular, the following modules could be considered off-the-shelf recommendation systems:
%\begin{itemize}
%\item Similar OSS projects: this recommendation concerns similar projects considering the libraries involved in the development. To this end, Crossim \cite{nguyen_crosssim:_2018} was proposed and implemented;
%\item API usage patterns: to provide the developer with useful API function calls, we developed and integrated FOCUS \cite{nguyen_focus:_2019} into the platform;
%\end{itemize}




